Denoising Task Routing for Diffusion Models

Diffusion models generate highly realistic images by learning a multi-step denoising process, naturally embodying the principles of multi-task learning (MTL). Despite the inherent connection between diffusion models and MTL, there remains an unexplored area in designing neural architectures that explicitly incorporate MTL into the framework of diffusion models. In this paper, we present Denoising Task Routing (DTR), a simple add-on strategy for existing diffusion model architectures to establish distinct information pathways for individual tasks within a single architecture by selectively activating subsets of channels in the model. What makes DTR particularly compelling is its seamless integration of prior knowledge of denoising tasks into the framework: (1) Task Affinity: DTR activates similar channels for tasks at adjacent timesteps and shifts activated channels as sliding windows through timesteps, capitalizing on the inherent strong affinity between tasks at adjacent timesteps. (2) Task Weights: During the early stages (higher timesteps) of the denoising process, DTR assigns a greater number of task-specific channels, leveraging the insight that diffusion models prioritize reconstructing global structure and perceptually rich contents in earlier stages, and focus on simple noise removal in later stages. Our experiments reveal that DTR not only consistently boosts diffusion models' performance across different evaluation protocols without adding extra parameters but also accelerates training convergence. Finally, we show the complementarity between our architectural approach and existing MTL optimization techniques, providing a more complete view of MTL in the context of diffusion training. Significantly, by leveraging this complementarity, we attain matched performance of DiT-XL using the smaller DiT-L with a reduction in training iterations from 7M to 2M.

==> algs/routing_mask_creation.tex <==
% \lstset{
%     language=C++,          % Set the programming language for syntax highlighting
%     basicstyle=\small\ttfamily, % Set the font and size for the code
%     numbers=left,          % Show line numbers on the left
%     numberstyle=\tiny,     % Set the style for line numbers
%     tabsize=4,             % Set the tab size
%     captionpos=b,          % Position of the caption (b=bottom)
%     breaklines=true,       % Automatically break lines if they're too long
%     frame=single,          % Add a frame around the code
%     showstringspaces=false % Don't show spaces in strings as underscores
% }

\algrenewcommand\algorithmicindent{0.5em}%
\begin{figure}[t]
\begin{minipage}[t]{0.495\textwidth}
\begin{algorithm}[H]
   \caption{\small{Random Masking (NumPy-like)}}
   \label{alg:random_mask}

    \definecolor{commentcolor}{rgb}{0.25,0.5,0.5}
    \definecolor{monokaigreen}{RGB}{166, 226, 46}
    \definecolor{monokaipurple}{RGB}{145, 94, 174}
    \definecolor{monokaired}{RGB}{255, 73, 85}
    \lstset{
        basicstyle=\fontsize{5.5pt}{5.5pt}\ttfamily\bfseries,
        commentstyle=\fontsize{5.5pt}{5.5pt}\color{commentcolor},
        keywordstyle=\fontsize{5.5pt}{5.5pt}\color{monokaipurple},
        stringstyle=\fontsize{5.5pt}{5.5pt}\color{monokaired},
        numbers=left,
        numberstyle=\tiny\color{gray},
        numbersep=-6pt,
        breaklines=true,
    }
    \begin{lstlisting}[language=python]
    # T: number of tasks
    # C: number of channels
    # alpha: channel shifting parameter
    # beta: activation ratio
    
    def random_masking(T, C, beta):
        # initialize mask with zeros
        mask = np.zeros(T, C)
        # number of activated channels
        num_activ = int(beta * C)
        # fill the mask with ones
        mask[:, : num_activ] = 1
        # randomly shuffle the columns of the mask    
        return mask[:, np.random.permutation(C)]
    \end{lstlisting}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}[t]{0.495\textwidth}
\begin{algorithm}[H]
   \caption{\small{DTR Masking (NumPy-like)}}
   \label{alg:dtr_mask}
   
    \definecolor{commentcolor}{rgb}{0.25,0.5,0.5}
    \definecolor{monokaigreen}{RGB}{166, 226, 46}
    \definecolor{monokaipurple}{RGB}{145, 94, 174}
    \definecolor{monokaired}{RGB}{255, 73, 85}
    \lstset{
        basicstyle=\fontsize{5.5pt}{5.5pt}\ttfamily\bfseries,
        commentstyle=\fontsize{5.5pt}{5.5pt}\color{commentcolor},
        keywordstyle=\fontsize{5.5pt}{5.5pt}\color{monokaipurple},
        stringstyle=\fontsize{5.5pt}{5.5pt}\color{monokaired},
        numbers=left,
        numberstyle=\tiny\color{gray},
        numbersep=-6pt,
        breaklines=true,
    }
    \begin{lstlisting}[language=python]
    def dtr_masking(T, C, alpha, beta):
        # initialize mask with zeros
        mask = np.zeros(T, C)
        # number of activated channels
        num_activ = int(beta * C)
        # number of deactivated channels
        num_deact = C - num_activ
        # create linearly spaced points 
        x = np.linspace(0, 1, T)
        # apply a scaling factor to linear points
        x = x ** alpha
        # calculate the channel offset for every timesteps
        offset = (num_deact * x).round()
        # fill the mask with ones
        for t in T:
            start = offset[t]
            end = offset[t] + num_activ
            mask[t, start:end] = 1
        return mask
    \end{lstlisting}
\end{algorithm}
\end{minipage}
\vspace{-6mm}
\end{figure}

==> figs/observation.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/observation.pdf}
    \caption{\textbf{Observation.}}
    \label{fig:observation}
\end{figure*}

==> figs/routing.tex <==
\begin{figure*}\centering
\includegraphics[width=\linewidth]{figs/routing.pdf}
\caption{\textbf{Routing architecture 설명.}}
\vspace{-2mm}
\label{fig:routing}\vspace{-2mm}
\end{figure*}

==> figs/t2i.tex <==
\providecommand{\imwidth}{}
\providecommand{\impath}[1]{}

\begin{figure*}[htbp]
\centering
	\renewcommand{\imwidth}{0.15\textwidth}
    \renewcommand{\impath}[1]{figs/##1}%
	\setlength{\tabcolsep}{1pt}
	\begin{tabular}{cccccc}
	\toprule
	\multicolumn{6}{c}{\small{Text-to-Image Synthesis on COCO 256$\times$256}} \\
	\midrule
    \shortstack{\tiny{\emph{'A street sign that reads}} \\ \tiny{\emph{``Latent Diffusion'' '}}} & \shortstack{\tiny{\emph{'A zombie in the}} \\ \tiny{\emph{style of Picasso'}}} & \shortstack{\tiny{\emph{'An image of an animal}} \\ \tiny{\emph{half mouse half octopus'}}} & \shortstack{\tiny{\emph{'An illustration of a slightly}} \\ \tiny{\emph{conscious neural network'}}} & \shortstack{\tiny{\emph{'A painting of a}} \\ \tiny{\emph{squirrel eating a burger'}}}  & \shortstack{\tiny{\emph{'A watercolor painting of a}} \\ \tiny{\emph{chair that looks like an octopus'}}} \\
	\midrule
	\includegraphics[align=c,width=\imwidth]{\impath{sample-3}} &
	\includegraphics[align=c,width=\imwidth]{\impath{sample-83}} &
	\includegraphics[align=c,width=\imwidth]{\impath{sample-50}} &
	\includegraphics[align=c,width=\imwidth]{\impath{sample-01}} &
	\includegraphics[align=c,width=\imwidth]{\impath{sample-0}} &
	\includegraphics[align=c,width=\imwidth]{\impath{sample-66}} \\
	
	\includegraphics[align=c,width=\imwidth]{\impath{sample-9}} &
	\includegraphics[align=c,width=\imwidth]{\impath{sample-91}} &
	\includegraphics[align=c,width=\imwidth]{\impath{sample-68}} &
	\includegraphics[align=c,width=\imwidth]{\impath{sample-09}} &
	\includegraphics[align=c,width=\imwidth]{\impath{sample-9}} &
	\includegraphics[align=c,width=\imwidth]{\impath{sample-83}} \\
	\bottomrule
	\end{tabular}
\caption{Samples for user-defined text prompts from our model for text-to-image synthesis, which was trained on the COCO~\cite{} database. \todo{Samples generated with 200 DDIM steps and $\eta = 1.0$. We use unconditional guidance \cite{ho2021classifier} with $s=10.0$.}}
\label{fig:t2i}
\end{figure*}

==> figs/training_speed.tex <==
\begin{figure*}[t]
\centering
\subfloat[Model Size (DiT)]{\includegraphics[width=0.32\linewidth]{figs/fast_convergence/model_size_convergence.png}}
\hspace{.05cm}
\subfloat[DiT with Loss Weighting]{\includegraphics[width=0.32\linewidth]{figs/fast_convergence/loss_convergence.png}}
\hspace{.05cm}
\subfloat[ADM]{\includegraphics[width=0.32\linewidth]{figs/fast_convergence/model_size_convergence.png}}
\vspace{-.2cm}
\caption{\textbf{Convergence comparison on ImageNet dataset.} We report FID-10K every 50$k$ iterations, excluding the results at the first 50K iterations.
}
\label{fig:training_speed}
\end{figure*}

==> tabs/imagenet.tex <==
\begin{table}[t]
    \begin{center}
    \begin{small}
    \scalebox{0.81}{
    \begin{tabular}{lccccc}
    \toprule
    \multicolumn{6}{l}{\bf{Class-Conditional ImageNet} 256$\times$256} \\
    \toprule
    Model & FID$\downarrow$   & sFID$\downarrow$  & IS$\uparrow$     & Precision$\uparrow$ & Recall$\uparrow$ \\
    \bottomrule
    BigGAN-deep~\cite{brock2018large} & 6.95 & 7.36 & 171.4 & 0.87 & 0.28 \\
    StyleGAN-XL~\cite{Sauer2021ARXIV} & 2.30 & 4.02 & 265.12 & 0.78 & 0.53 \\
    \toprule
    ADM~\cite{dhariwal2021adm} & 10.94 & 6.02 & 100.98 & 0.69 & 0.63 \\
    ADM-U & 7.49 & 5.13 & 127.49 & 0.72 & 0.63 \\
    ADM-G & 4.59 & 5.25 & 186.70 & 0.82 & 0.52 \\
    ADM-G, ADM-U & 3.94 & 6.14      & 215.84 & 0.83 & 0.53 \\
    \arrayrulecolor{gray}\cmidrule(lr){1-6}
    CDM~\cite{ho2021cascaded} & 4.88 & - & 158.71 & - & - \\
    \arrayrulecolor{gray}\cmidrule(lr){1-6}
    LDM-8~\cite{rombach2021highresolution} & 15.51 & - & 79.03 & 0.65 & 0.63 \\
    LDM-8-G & 7.76 & - & 209.52 & 0.84 & 0.35 \\
    LDM-4 & 10.56 & - & 103.49 & 0.71 & 0.62 \\
    LDM-4-G (cfg=1.25) &  3.95 & - & 178.22 & 0.81 & 0.55 \\
    LDM-4-G (cfg=1.50) & 3.60 & - & 247.67 & \textbf{0.87} & 0.48 \\
    \arrayrulecolor{gray}\cmidrule(lr){1-6}
    \textbf{DiT-XL/2}              & 9.62 & 6.85 & 121.50 & 0.67 & \textbf{0.67} \\
    \textbf{DiT-XL/2-G} (cfg=1.25) & 3.22 & 5.28 & 201.77 & 0.76 & 0.62 \\
    \textbf{DiT-XL/2-G} (cfg=1.50) & \textbf{2.27} & \textbf{4.60} & \textbf{278.24} & 0.83 & 0.57 \\
    \bottomrule
    \end{tabular}
    } %
    \end{small}
    \end{center}
    \vspace{-4mm}
    \caption{\textbf{Benchmarking class-conditional image generation on ImageNet 256$\times$256.} DiT-XL/2 achieves state-of-the-art FID.} %
    \label{tab:imagenet}
\end{table}

==> tabs/routing_arch_abl.tex <==
\begin{table*}[t]
    \begin{center}
    \begin{small}
    \scalebox{1.0}{
    \begin{tabular}{lccccc}
    \toprule
    \multicolumn{5}{l}{\bf{Class-Conditional ImageNet} 256$\times$256} \\
    \toprule
    Moel & Design & FID$\downarrow$  & IS$\uparrow$  & Precision$\uparrow$ & Recall$\uparrow$ \\
    \toprule
    \multirow{3}{*}{ADM~\citep{dhariwal2021diffusion}} & baseline & - & - & - & -  \\
                                                       & skip-connection & - & - & - & -  \\
                                                       & GroupNorm & - & - & - & - \\
    \arrayrulecolor{gray}\cmidrule(lr){1-6}
    \multirow{3}{*}{DiT~\citep{peebles2022scalable}}   & baseline & - & - & - & -  \\
                                                       & skip-connection & - & - & - & -  \\
                                                       & Attn-MLP & - & - & - & - \\
    \bottomrule
    \toprule
    \multicolumn{5}{l}{\bf{Text-Conditional MS-COCO} 256$\times$256} \\
    \toprule
    Moel & Design & FID$\downarrow$  & IS$\uparrow$  & Precision$\uparrow$ & Recall$\uparrow$ \\    
    \toprule
    \multirow{4}{*}{DiT~\citep{peebles2022scalable}}   & pooled condition & - & - & - & -  \\
                                                       & cross-self-mlp & - & - & - & - \\
                                                       & self-cross-mlp & - & - & - & - \\
                                                       & self-mlp-cross & - & - & - & - \\
    \bottomrule
    \end{tabular}
    }
    \end{small}
    \end{center}
    \vspace{-4mm}
    \caption{\textbf{Routing Architecture Ablation on ImageNet 256$\times$256.} Cosine Scheduling.} %
    \label{tab:routing_arch_abl}
\end{table*}

